Better Summarization Evaluation with Word Embeddings for ROUGE

ROUGE is a widely adopted, automatic evaluation measure for text summarization. While it has been shown to correlate well with human judgements, it is biased towards surface lexical similarities. This makes it unsuitable for the evaluation of abstractive summarization, or summaries with substantial paraphrasing. We study the effectiveness of word embeddings to overcome this disadvantage of ROUGE. Specifically, instead of measuring lexical overlaps, word embeddings are used to compute the semantic similarity of the words used in summaries instead. Our experimental results show that our proposal is able to achieve better correlations with human judgements when measured with the Spearman and Kendall rank coefficients.

==> 500_discussion.tex <==
We believe that the results we have shown in this work so far show that the use of word embeddings as we have proposed, can help to enhance the evaluation performance of ROUGE.
However, what is also clear from our experiments here is that the AESOP dataset and the use of the various correlation measures may not be sufficient to help us properly assess and compare new automatic evaluation measures.

To further validate the efficacy of our proposal (or any proposed automatic evaluation measure for that matter), it will be helpful to expand on the collection of summaries collected in the AESOP dataset.
In particular, these summaries are derived from systems participating in the TAC summarization task, where there is a strong exhibited bias towards extractive summarizers.
It will be helpful to enlarge this set of summaries to include output from summarizers which carry out substantial paraphrasing~\cite{ng2014_timeline,li2013document}, or abstractive summarizers~\cite{liu2015_abstractive}.

We also like to point out for completeness that the correlation of the automatic measures for pyramid and responsiveness are much better than for readability. 
The original ROUGE measures, and accordingly, our proposed \texttt{ROUGE-WE}, make no provision to cater for fluency.
They are designed to capture content similarity much better than the fluency and coherence of the generated summaries.
As such as have avoided a more thorough analysis of the results we see in Table~\ref{tab:results_main_fl}.

\subsection{Future Work}

We want to build on this work in two key ways.
First, we want to examine the utility of word embeddings in greater detail.
We mentioned earlier that it is straight forward to extend our similarity function $f_{WE}$ to incorporate n-grams and skip-n-grams.
To achieve this, we will also need to update the training data used by \texttt{word2vec} so that we can still keep the number of out-of-vocabulary words to an acceptable level.
Along the same line, we can also expand on the concept of word embeddings, and attempt to convert sentences into vector representations also such as in \newcite{le2014_sentvect}.

Next, we hope to improve on the objective measures we have of summarization systems.
As seen in our experimental results, the existing evaluation methodology in AESOP may give rise to inconsistencies. 
Further, it draws on a limited set of summarization systems which may not be sufficiently diverse.
%Existing work is very useful for tweet summarization evaluation
%- common metric due to short length of summaries

%Future work
%
%Extending this to ROUGE-2 and beyond
%- Need better word2vec training
%- Challenges
%
%Looking at sentence 2 vec
% 


